CMB-S4 Science Book, First Edition

This book lays out the scientific goals to be addressed by the next-generation ground-based cosmic microwave background experiment, CMB-S4, envisioned to consist of dedicated telescopes at the South Pole, the high Chilean Atacama plateau and possibly a northern hemisphere site, all equipped with new superconducting cameras. CMB-S4 will dramatically advance cosmological studies by crossing critical thresholds in the search for the B-mode polarization signature of primordial gravitational waves, in the determination of the number and masses of the neutrinos, in the search for evidence of new light relics, in constraining the nature of dark energy, and in testing general relativity on large scales.

==> Inflation/forecast_cmbs4.tex <==
%%%%%% CMB-S4 Inflation Chapter  %%%%%%%%%%%%%%%%
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Forecasts}
\label{sec:forecasts}
(Jo is checking she can use git)


==> affil_defs.tex <==
\newcounter{affilcount}
\stepcounter{affilcount}

\def\Irvinetext{University of California, Irvine}
\def\Irvine{\value{affilcount}}
\stepcounter{affilcount}

\def\Illtext{University of Illinois, Urbana-Champaign}
\def\Ill{\value{affilcount}}
\stepcounter{affilcount}

\def\Penntext{University of Pennsylvania}
\def\Penn{\value{affilcount}}
\stepcounter{affilcount}

\def\Slactext{SLAC National Accelerator Laboratory}
\def\Slac{\value{affilcount}}
\stepcounter{affilcount}

\def\Princetontext{Princeton University}
\def\Princeton{\value{affilcount}}
\stepcounter{affilcount}

\def\Hopkinstext{Johns Hopkins University}
\def\Hopkins{\value{affilcount}}
\stepcounter{affilcount}

\def\Stanfordtext{Stanford University}
\def\Stanford{\value{affilcount}}
\stepcounter{affilcount}

\def\Oxfordtext{University of Oxford, United Kingdom}
\def\Oxford{\value{affilcount}}
\stepcounter{affilcount}

\def\Fermitext{Fermilab National Accelerator Laboratory}
\def\Fermi{\value{affilcount}}
\stepcounter{affilcount}

\def\Chicagotext{University of Chicago}
\def\Chicago{\value{affilcount}}
\stepcounter{affilcount}

\def\Sandiegotext{University of California, San Diego}
\def\Sandiego{\value{affilcount}}
\stepcounter{affilcount}

\def\Nisttext{National Institute of Standards and Technology}
\def\Nist{\value{affilcount}}
\stepcounter{affilcount}

\def\Sissatext{Scuola Internazionale Superiore di Studi Avanzati, Trieste, Italy}
\def\Sissa{\value{affilcount}}
\stepcounter{affilcount}

\def\Berkeleytext{University of California, Berkeley}
\def\Berkeley{\value{affilcount}}
\stepcounter{affilcount}

\def\Apctext{Laboratoire AstroParticule et Cosmologie - Université Paris Diderot, France}
\def\Apc{\value{affilcount}}
\stepcounter{affilcount}

\def\Iaptext{Institut d'Astrophysique de Paris - Université Pierre et Marie Curie /  Centre National de la Recherche Scientifique, France}
\def\Iap{\value{affilcount}}
\stepcounter{affilcount}

\def\Anltext{Argonne National Laboratory}
\def\Anl{\value{affilcount}}
\stepcounter{affilcount}

\def\Cincytext{University of Cincinnati}
\def\Cincy{\value{affilcount}}
\stepcounter{affilcount}

\def\Citatext{Canadian Institute For Theoretical Astrophysics, Canada}
\def\Cita{\value{affilcount}}
\stepcounter{affilcount}

\def\Lbnltext{Lawrence Berkeley National Laboratory}
\def\Lbnl{\value{affilcount}}
\stepcounter{affilcount}

\def\Manchestertext{University of Manchester, United Kingdom}
\def\Manchester{\value{affilcount}}
\stepcounter{affilcount}

\def\Perimetertext{Perimeter Institute, Canada}
\def\Perimeter{\value{affilcount}}
\stepcounter{affilcount}

\def\Harvardtext{Harvard University}
\def\Harvard{\value{affilcount}}
\stepcounter{affilcount}

\def\Sapienziatext{Sapienza - Università di Roma, Italy}
\def\Sapienzia{\value{affilcount}}
\stepcounter{affilcount}

\def\Dartmouthtext{Dartmouth College}
\def\Dartmouth{\value{affilcount}}
\stepcounter{affilcount}

\def\Kwazulutext{University of KwaZulu-Natal, South Africa}
\def\Kwazulu{\value{affilcount}}
\stepcounter{affilcount}

\def\Novatext{Villanova University}
\def\Nova{\value{affilcount}}
\stepcounter{affilcount}

\def\Cornelltext{Cornell University}
\def\Cornell{\value{affilcount}}
\stepcounter{affilcount}

\def\Jpltext{Jet Propulsion Laboratory}
\def\Jpl{\value{affilcount}}
\stepcounter{affilcount}

\def\Caltechtext{California Institute of Technology}
\def\Caltech{\value{affilcount}}
\stepcounter{affilcount}

\def\Cnrstext{Centre National de la Recherche Scientifique, France}
\def\Cnrs{\value{affilcount}}
\stepcounter{affilcount}

\def\Penntext{University of Pennsylvania}
\def\Penn{\value{affilcount}}
\stepcounter{affilcount}

\def\Arcetritext{Istituto Nazionale di Astrofisica - Osservatorio Astrofisico di Arcetri, Italy}
\def\Arcetri{\value{affilcount}}
\stepcounter{affilcount}

\def\Mcgilltext{McGill University, Canada}
\def\Mcgill{\value{affilcount}}
\stepcounter{affilcount}

\def\Ilptext{Institut Lagrange Paris - Université Pierre et Marie Curie /  Centre National de la Recherche Scientifique, France}
\def\Ilp{\value{affilcount}}
\stepcounter{affilcount}

\def\Ccatext{Center for Computational Astrophysics}
\def\Cca{\value{affilcount}}
\stepcounter{affilcount}

\def\Muddtext{Harvey Mudd College}
\def\Mudd{\value{affilcount}}
\stepcounter{affilcount}

\def\Icetext{Institut de Ciències de l'Espai, Spain}
\def\Ice{\value{affilcount}}
\stepcounter{affilcount}

\def\Stockholmtext{Stockholm University, Sweden}
\def\Stockholm{\value{affilcount}}
\stepcounter{affilcount}

\def\Iastext{Institute for Advanced Study}
\def\Ias{\value{affilcount}}
\stepcounter{affilcount}

\def\Haverfordtext{Haverford College}
\def\Haverford{\value{affilcount}}
\stepcounter{affilcount}

\def\Michigantext{University of Michigan}
\def\Michigan{\value{affilcount}}
\stepcounter{affilcount}

\def\Ubctext{University of British Columbia, Canada}
\def\Ubc{\value{affilcount}}
\stepcounter{affilcount}

\def\Bouldertext{University of Colorado Boulder}
\def\Boulder{\value{affilcount}}
\stepcounter{affilcount}

\def\Minnesotatext{University of Minnesota}
\def\Minnesota{\value{affilcount}}
\stepcounter{affilcount}

\def\Laltext{Laboratoire de l'Accélérateur Linéaire, France}
\def\Lal{\value{affilcount}}
\stepcounter{affilcount}

\def\Columbiatext{Columbia University}
\def\Columbia{\value{affilcount}}
\stepcounter{affilcount}

\def\Osutext{The Ohio State University}
\def\Osu{\value{affilcount}}
\stepcounter{affilcount}

\def\Torontotext{University of Toronto, Canada}
\def\Toronto{\value{affilcount}}
\stepcounter{affilcount}

\def\Fsutext{Florida State University}
\def\Fsu{\value{affilcount}}
\stepcounter{affilcount}

\def\Davistext{University of California, Davis}
\def\Davis{\value{affilcount}}
\stepcounter{affilcount}

\def\Pitttext{University of Pittsburgh}
\def\Pitt{\value{affilcount}}
\stepcounter{affilcount}

\def\Ferraratext{Università di Ferrara, Italy}
\def\Ferrara{\value{affilcount}}
\stepcounter{affilcount}

\def\Sussextext{University of Sussex, United Kingdom}
\def\Sussex{\value{affilcount}}
\stepcounter{affilcount}

\def\Stonytext{Stony Brook University}
\def\Stony{\value{affilcount}}
\stepcounter{affilcount}

\def\Madisontext{University of Wisconsin - Madison}
\def\Madison{\value{affilcount}}
\stepcounter{affilcount}

\def\Santabarbaratext{University of California, Santa Barbara}
\def\Santabarbara{\value{affilcount}}
\stepcounter{affilcount}

\def\Lpsctext{Laboratoire de Physique Subatomique & Cosmologie - Institut national de physique nucléaire et de physique des particules (Centre National de la Recherche Scientifique) / Université Grenoble Alpes}
\def\Lpsc{\value{affilcount}}
\stepcounter{affilcount}

\def\Kingstext{King's College London, United Kingdom}
\def\Kings{\value{affilcount}}
\stepcounter{affilcount}

\def\Asutext{Arizona State University}
\def\Asu{\value{affilcount}}
\stepcounter{affilcount}

\def\Ceatext{Commissariat à l'Energie Atomique - Saclay, France}
\def\Cea{\value{affilcount}}
\stepcounter{affilcount}

\def\Usctext{University of Southern California}
\def\Usc{\value{affilcount}}
\stepcounter{affilcount}

\def\Bohrtext{Niels Bohr Institute, Denmark}
\def\Bohr{\value{affilcount}}
\stepcounter{affilcount}

\def\Orsaytext{Institut d'Astrophysique Spatiale - Orsay, France}
\def\Orsay{\value{affilcount}}
\stepcounter{affilcount}

\def\Sfutext{Simon Fraser University, Canada}
\def\Sfu{\value{affilcount}}
\stepcounter{affilcount}

\def\Oslotext{University of Oslo, Norway}
\def\Oslo{\value{affilcount}}
\stepcounter{affilcount}

\def\Melbournetext{University of Melbourne, Australia}
\def\Melbourne{\value{affilcount}}
\stepcounter{affilcount}

\def\Casetext{Case Western Reserve University}
\def\Case{\value{affilcount}}
\stepcounter{affilcount}

\def\Pennstatetext{The Pennsylvania State University}
\def\Pennstate{\value{affilcount}}
\stepcounter{affilcount}

\def\Brookhaventext{Brookhaven National Laboratory}
\def\Brookhaven{\value{affilcount}}
\stepcounter{affilcount}

\def\Swarthmoretext{Swarthmore College}
\def\Swarthmore{\value{affilcount}}
\stepcounter{affilcount}

\def\Hpdtext{High Precision Devices, Boulder, CO}
\def\Hpd{\value{affilcount}}
\stepcounter{affilcount}

\def\Umasstext{University of Massachusetts, Amherst}
\def\Umass{\value{affilcount}}
\stepcounter{affilcount}

\def\Iucaatext{Inter-University Centre for Astronomy and Astrophysics, India}
\def\Iucaa{\value{affilcount}}
\stepcounter{affilcount}

\def\Saotext{Smithsonian Astrophysical Observatory}
\def\Sao{\value{affilcount}}
\stepcounter{affilcount}

\def\Mittext{Massachusetts Institute of Technology}
\def\Mit{\value{affilcount}}
\stepcounter{affilcount}

\def\Browntext{Brown University}
\def\Brown{\value{affilcount}}
\stepcounter{affilcount}

\def\Syracusetext{Syracuse University}
\def\Syracuse{\value{affilcount}}
\stepcounter{affilcount}

\def\Gsfctext{National Aeronautics and Space Administration Goddard Space Flight Center}
\def\Gsfc{\value{affilcount}}
\stepcounter{affilcount}



==> contributor_list.tex <==
\begin{center}
\textbf{List of Contributors}
\end{center}
Kevork N.~Abazajian (University of California, Irvine),
Peter Adshead (University of Illinois, Urbana-Champaign),
Zeeshan Ahmed (SLAC National Accelerator Laboratory),
Steven W.~Allen (Stanford),
David Alonso (University of Oxford),
Kam S.~Arnold (University of California, San Diego),
Carlo Baccigalupi (SISSA),
James G.~Bartlett (APC - Université Paris Diderot),
Nicholas Battaglia (Princeton University),
Bradford A.~Benson (Fermilab),
Colin A.~Bischoff (University of Cincinnati),
Julian Borrill (Berkeley Lab),
Victor Buza (Harvard University),
Erminia Calabrese (University of Oxford),
Robert Caldwell (Dartmouth College),
John E.~Carlstrom (University of Chicago),
Clarence L.~Chang (Argonne National Laboratory),
Thomas M.~Crawford (University of Chicago),
Francis-Yan Cyr-Racine (Department of Physics, Harvard University),
Francesco De Bernardis (Cornell University),
Tijmen de Haan (UC Berkeley),
Sperello di Serego Alighieri (INAF - Osservatorio Astrofisico di Arcetri),
Joanna Dunkley (Princeton University),
Cora Dvorkin (Harvard University),
Josquin Errard (Institut Lagrange Paris),
Giulio Fabbian (SISSA),
Stephen Feeney (Center for Computational Astrophysics),
Simone Ferraro (University of California, Berkeley),
Jeffrey P.~Filippini (University of Illinois at Urbana-Champaign),
Raphael Flauger (University of California, San Diego),
George M.~Fuller (University of California, San Diego),
Vera Gluscevic (Institute for Advanced Study),
Daniel Green (UC Berkeley),
Daniel Grin (Haverford College),
Evan Grohs (University of Michigan),
Jason W.~Henning (University of Chicago),
J. Colin Hill (Columbia University),
Ren\'{e}e Hlo\v{z}ek (Dunlap Institute),
Gilbert Holder (University of Illinois at Urbana-Champaign),
William Holzapfel (University of California),
Wayne Hu (University of Chicago),
Kevin M.~Huffenberger (Florida State University),
Reijo Keskitalo (Lawrence Berkeley Lab),
Lloyd Knox (UC Davis),
Arthur Kosowsky (University of Pittsburgh),
John Kovac (Harvard University),
Ely D.~Kovetz (Johns Hopkins University),
Chao-Lin Kuo (SLAC),
Akito Kusaka (Lawrence Berkeley National Laboratory),
Maude Le Jeune (APC, Univ Paris Diderot),
Adrian T.~Lee (University of California, Berkeley),
Marc Lilley (IAP),
Marilena Loverde (Stony Brook University),
Mathew S.~Madhavacheril (Princeton University),
Adam Mantz (Stanford University),
David J.~E.~Marsh (King's College London),
Jeffrey McMahon (University of Michigan),
Pieter Daniel Meerburg (CITA),
Joel Meyers (CITA),
Amber D.~Miller (University of Southern California),
Julian B.~Munoz (Johns Hopkins University),
Ho Nam Nguyen (Stony Brook University),
Michael D.~Niemack (Cornell University),
Marco Peloso (University of Minnesota),
Julien Peloton (University of Sussex),
Levon Pogosian (Simon Fraser University),
Clement Pryke (University of Minnesota),
Marco Raveri (University of Chicago),
Christian L.~Reichardt (The University of Melbourne),
Graca Rocha (Jet Propulsion Laboratory),
Aditya Rotti (Florida State University),
Emmanuel Schaan (Princeton University),
Marcel M.~Schmittfull (UC Berkeley),
Douglas Scott (University of British Columbia),
Neelima Sehgal (Stony Brook University),
Sarah Shandera (The Pennsylvania State University),
Blake D. Sherwin (University of California, Berkeley),
Tristan L.~Smith (Swarthmore College),
Lorenzo Sorbo (University of Massachusetts, Amherst),
Glenn D.~Starkman (Case Western Reserve University),
Kyle T.~Story (Stanford),
Alexander van Engelen (CITA),
Joaquin D.~Vieira (University of Illinois at Urbana-Champaign),
Scott Watson (Syracuse University),
Nathan Whitehorn (UC Berkeley),
W.~L.~Kimmy Wu (UC Berkeley).


==> endorser_list.tex <==
\begin{center}
\textbf{List of Endorsers}
\end{center}

The following people have endorsed the science case for CMB-S4 as presented here and many of them have contributed directly to the writing of this document:

Kevork N.~Abazajian (University of California, Irvine),
Peter Adshead (University of Illinois, Urbana-Champaign),
James Aguirre (University of Pennsylvania),
Zeeshan Ahmed (SLAC National Accelerator Laboratory),
Simone Aiola (Princeton University),
Yacine Ali-Haimoud (Johns Hopkins University),
Steven W.~Allen (Stanford),
David Alonso (University of Oxford),
Adam Anderson (Fermilab),
James Annis (Fermilab),
John W.~Appel (Johns Hopkins University),
Douglas E.~Applegate (University of Chicago),
Kam S.~Arnold (University of California, San Diego),
Jason E.~Austermann (NIST),
Carlo Baccigalupi (SISSA),
Darcy Barron (UC Berkeley),
James G.~Bartlett (APC - Université Paris Diderot),
Ritoban Basu Thakur (KICP),
Nicholas Battaglia (Princeton University),
Daniel Baumann (Cambridge University),
Karim Benabed (Institut d'Astrophysique de Paris - UPMC/CNRS),
Amy N.~Bender (Argonne National Laboratory),
Charles L.~Bennett (Johns Hopkins University),
Bradford A.~Benson (Fermilab),
Colin A.~Bischoff (University of Cincinnati),
Lindsey Bleem (Argonne National Laboratory),
J.~Richard Bond (Canadian Institute For Theoretical Astrophysics),
Julian Borrill (Berkeley Lab),
François R.~Bouchet (Institut d'Astrophysique de Paris),
Michael L.~Brown (University of Manchester),
Christopher Brust (Perimeter Institute),
Victor Buza (Harvard University),
Karen Byrum (Argonne National Laboratory),
Giovanni Cabass (University of Rome La Sapienza),
Erminia Calabrese (University of Oxford),
Robert Caldwell (Dartmouth College),
John E.~Carlstrom (University of Chicago),
Anthony Challinor (University of Cambridge),
Clarence L.~Chang (Argonne National Laboratory),
Hsin C.~Chiang (University of KwaZulu-Natal),
David T.~Chuss (Villanova University),
Asantha Cooray (University of California, Irvine),
Nicholas F.~Cothard (Cornell University),
Thomas M.~Crawford (University of Chicago),
Brendan Crill (Jet Propulsion Laboratory),
Abigail Crites (Caltech),
Francis-Yan Cyr-Racine (Department of Physics, Harvard University),
Francesco De Bernardis (Cornell University),
Paolo M.~de Bernardis (Physics Department Sapienza University),
Tijmen de Haan (UC Berkeley),
Jacques Delabrouille (CNRS / APC),
Marcel Demarteau (Argonne National Laboratory),
Mark Devlin (University of Pennsylvania),
Sperello di Serego Alighieri (INAF - Osservatorio Astrofisico di Arcetri),
Eleonora di Valentino (IAP),
Clive Dickinson (The University of Manchester),
Matt Dobbs (McGill University),
Scott Dodelson (Fermilab),
Olivier Dore (JPL/Caltech),
Joanna Dunkley (Princeton University),
Cora Dvorkin (Harvard University),
Josquin Errard (Institut Lagrange Paris),
Thomas Essinger-Hileman (Johns Hopkins University), 
Giulio Fabbian (SISSA),
Stephen Feeney (Center for Computational Astrophysics),
Simone Ferraro (University of California, Berkeley),
Jeffrey P.~Filippini (University of Illinois at Urbana-Champaign),
Raphael Flauger (University of California, San Diego),
Aurelien A.~Fraisse (Princeton University),
George M.~Fuller (University of California, San Diego),
Patricio A.~Gallardo (Department of Physics, Cornell University.),
Silvia Galli (Institut d'Astrophysique de Paris),
Jason Gallicchio (Harvey Mudd),
Ken Ganga (APC),
Enrique Gaztanaga (Institute of Space Sciences),
Martina Gerbino (OKC, Stockholm University),
Mandeep S.~S.~Gill (Stanford),
Yannick Giraud-Héraud (APC - France),
Vera Gluscevic (Institute for Advanced Study),
Sunil Golwala (Caltech),
Krzysztof M.~Gorski (Jet Propulsion Laboratory),
Daniel Green (UC Berkeley),
Daniel Grin (Haverford College),
Evan Grohs (University of Michigan),
Riccardo Gualtieri (University of Illinois at Urbana Champaign),
Jon E.~Gudmundsson (Stockholm University),
Grantland Hall (Harvard University),
Mark Halpern (University of British Columbia),
Nils W.~Halverson (University of Colorado Boulder),
Shaul Hanany (University of Minnesota),
Shawn Henderson (Cornell University),
Jason W.~Henning (University of Chicago),
Sophie Henrot-Versille (LAL),
Sergi R.~Hildebrandt (California Institute of Technology),
J. Colin Hill (Columbia University),
Christopher M.~Hirata (The Ohio State University),
Eric Hivon (IAP),
Ren\'{e}e Hlo\v{z}ek (Dunlap Institute),
Gilbert Holder (University of Illinois at Urbana-Champaign),
William Holzapfel (University of California),
Wayne Hu (University of Chicago),
Johannes Hubmayr (NIST),
Kevin M.~Huffenberger (Florida State University),
Kent Irwin (Stanford),
Bradley R.~Johnson (Columbia University),
William C.~Jones (Princeton University),
Marc Kamionkowski (Johns Hopkins University),
Brian Keating (University of California, San Diego),
Sarah Kernasovskiy (Stanford University),
Reijo Keskitalo (Lawrence Berkeley Lab),
Theodore Kisner (Lawrence Berkeley National Laboratory),
Lloyd Knox (UC Davis),
Brian J.~Koopman (Cornell University),
Arthur Kosowsky (University of Pittsburgh),
John Kovac (Harvard University),
Ely D.~Kovetz (Johns Hopkins University),
Nicoletta Krachmalnicoff (SISSA),
Chao-Lin Kuo (SLAC),
Akito Kusaka (Lawrence Berkeley National Laboratory),
Nicole A.~Larsen (University of Chicago),
Massimiliano Lattanzi (Università di Ferrara),
Charles R.~Lawrence (JPL),
Maude Le Jeune (APC, Univ Paris Diderot),
Adrian T.~Lee (University of California, Berkeley),
Antony Lewis (University of Sussex),
Marc Lilley (IAP),
Thibaut Louis (IAP),
Marilena Loverde (Stony Brook University),
Amy Lowitz (University of Wisconsin - Madison),
Philip M.~Lubin (UC Santa Barbara - Physics),
Juan J.~F.~Macias-Perez (LPSC),
Mathew S.~Madhavacheril (Princeton University),
Adam Mantz (Stanford University),
David J.~E.~Marsh (King's College London),
Silvia R.~M.~Masi (Physics Department Sapienza University),
Philip Mauskopf (Arizona State University),
Jeffrey McMahon (University of Michigan),
Pieter Daniel Meerburg (CITA),
Alessandro Melchiorri (University of Rome Sapienza),
Jean-Baptiste Melin (CEA Saclay),
Stephan Meyer (University of Chicago),
Joel Meyers (CITA),
Amber D.~Miller (University of Southern California),
Laura M.~Mocanu (University of Chicago),
Lorenzo Moncelsi (California Institute of Technology),
Julian B.~Munoz (Johns Hopkins University),
Andrew Nadolski (University of Illinois, Urbana-Champaign),
Pavel Naselsky (Niels Bohr Institute),
Paolo Natoli (University of Ferrara),
Ho Nam Nguyen (Stony Brook University),
Michael D.~Niemack (Cornell University),
Stephen Padin (University of Chicago),
Luca Pagano (IAS - Orsay),
Lyman Page (Princeton University),
Robert Bruce Partridge (Haverford College),
Guillaume Patanchon (APC - France),
Timothy J.~Pearson (Caltech),
Marco Peloso (University of Minnesota),
Julien Peloton (University of Sussex),
Olivier Perdereau (LAL),
Laurence Perotto (LPSC-CNRS-France),
Francesco Piacentini (Sapienza - University of Rome),
Michel Piat (APC - France),
Levon Pogosian (Simon Fraser University),
Clement Pryke (University of Minnesota),
Benjamin Racine (University of Oslo),
Srinivasan Raghunathan (University of Melbourne),
Alexandra Rahlin (Fermilab),
Marco Raveri (University of Chicago),
Christian L.~Reichardt (The University of Melbourne),
Mathieu Remazeilles (University of Manchester),
Graca Rocha (Jet Propulsion Laboratory),
Natalie A.~Roe (LBNL),
Aditya Rotti (Florida State University),
John Ruhl (Case Western Reserve University),
Laura Salvati (University of Rome, Sapienza),
Emmanuel Schaan (Princeton University),
Marcel M.~Schmittfull (UC Berkeley),
Douglas Scott (University of British Columbia),
Neelima Sehgal (Stony Brook University),
Sarah Shandera (The Pennsylvania State University),
Christopher Sheehy (Brookhaven National Laboratory),
Blake D. Sherwin (University of California, Berkeley),
Erik Shirokoff (University of Chicago),
Eva Silverstein (Stanford University),
Sara M.~Simon (University of Michigan),
Tristan L.~Smith (Swarthmore College),
Michael Snow (High Precision Devices),
Lorenzo Sorbo (University of Massachusetts, Amherst),
Tarun Souradeep (IUCAA),
Suzanne T.~Staggs (Princeton University),
Antony A.~Stark (Smithsonian Astrophysical Observatory),
Glenn D.~Starkman (Case Western Reserve University),
George F.~Stein (Canadian Institute for Theoretical Astrophysics),
Jason R.~Stevens (Cornell),
Radek Stompor (APC/France),
Kyle T.~Story (Stanford),
Chris Stoughton (Fermilab),
Meng Su (MIT),
Aritoki Suzuki (University of California, Berkeley),
Grant P.~Teply (University of California, San Diego),
Peter Timbie (UW-Madison),
Jesse I.~Treu (Princeton University),
Matthieu Tristram (LAL - CNRS),
Gregory Tucker (Brown University),
Sunny Vagnozzi (Stockholm University),
Alexander van Engelen (CITA),
Eve M.~Vavagiakis (Cornell University),
Joaquin D.~Vieira (University of Illinois at Urbana-Champaign),
Abigail G.~Vieregg (University of Chicago, Dept. of Physics),
Sebastian von Hausegger (Niels Bohr Institute),
Benjamin D.~Wandelt (Institut d'Astrophysique de Paris),
Scott Watson (Syracuse University),
Nathan Whitehorn (UC Berkeley),
Edward J.~Wollack (NASA Goddard Space Flight Center),
W.~L.~Kimmy Wu (UC Berkeley),
Zhilei Xu (Johns Hopkins University),
Ki Won Yoon (SLAC),
Matias Zaldarriaga (Institute for Advanced Study).


==> endorser_list_indexed_orig.tex <==
\newcounter{affilcount}

\newcommand{\affil}[1]{\refstepcounter{affilcount}\label{#1}}

\def\Irvinetext{University of California, Irvine}
\affil{Irvine}
\def\Illtext{University of Illinois, Urbana-Champaign}
\affil{Ill}
\def\Penntext{University of Pennsylvania}
\affil{Penn}
\def\Slactext{SLAC National Accelerator Laboratory}
\affil{Slac}
\def\Princetontext{Princeton University}
\affil{Princeton}
\def\Hopkinstext{Johns Hopkins University}
\affil{Hopkins}
\def\Stanfordtext{Stanford University}
\affil{Stanford}
\def\Oxfordtext{University of Oxford, United Kingdom}
\affil{Oxford}
\def\Fermitext{Fermilab National Accelerator Laboratory}
\affil{Fermi}
\def\Chicagotext{University of Chicago}
\affil{Chicago}
\def\Sandiegotext{University of California, San Diego}
\affil{Sandiego}
\def\Nisttext{National Institute of Standards and Technology}
\affil{Nist}
\def\Sissatext{Scuola Internazionale Superiore di Studi Avanzati, Trieste, Italy}
\affil{Sissa}
\def\Berkeleytext{University of California, Berkeley}
\affil{Berkeley}
\def\Apctext{Laboratoire AstroParticule et Cosmologie - Université Paris Diderot, France}
\affil{Apc}
\def\Cambridgetext{University of Cambridge, United Kingdom}
\affil{Cambridge}
\def\Iaptext{Institut d'Astrophysique de Paris - Université Pierre et Marie Curie /  Centre National de la Recherche Scientifique, France}
\affil{Iap}
\def\Anltext{Argonne National Laboratory}
\affil{Anl}
\def\Cincytext{University of Cincinnati}
\affil{Cincy}
\def\Citatext{Canadian Institute For Theoretical Astrophysics, Canada}
\affil{Cita}
\def\Lbnltext{Lawrence Berkeley National Laboratory}
\affil{Lbnl}
\def\Manchestertext{University of Manchester, United Kingdom}
\affil{Manchester}
\def\Perimetertext{Perimeter Institute, Canada}
\affil{Perimeter}
\def\Harvardtext{Harvard University}
\affil{Harvard}
\def\Sapienzatext{Sapienza - Università di Roma, Italy}
\affil{Sapienza}
\def\Dartmouthtext{Dartmouth College}
\affil{Dartmouth}
\def\Kwazulutext{University of KwaZulu-Natal, South Africa}
\affil{Kwazulu}
\def\Novatext{Villanova University}
\affil{Nova}
\def\Cornelltext{Cornell University}
\affil{Cornell}
\def\Jpltext{Jet Propulsion Laboratory}
\affil{Jpl}
\def\Caltechtext{California Institute of Technology}
\affil{Caltech}
\def\Cnrstext{Centre National de la Recherche Scientifique, France}
\affil{Cnrs}
\def\Arcetritext{Istituto Nazionale di Astrofisica - Osservatorio Astrofisico di Arcetri, Italy}
\affil{Arcetri}
\def\Mcgilltext{McGill University, Canada}
\affil{Mcgill}
\def\Ilptext{Institut Lagrange Paris - Université Pierre et Marie Curie /  Centre National de la Recherche Scientifique, France}
\affil{Ilp}
\def\Ccatext{Center for Computational Astrophysics}
\affil{Cca}
\def\Muddtext{Harvey Mudd College}
\affil{Mudd}
\def\Icetext{Institut de Ciències de l'Espai, Spain}
\affil{Ice}
\def\Stockholmtext{Stockholm University, Sweden}
\affil{Stockholm}
\def\Iastext{Institute for Advanced Study}
\affil{Ias}
\def\Haverfordtext{Haverford College}
\affil{Haverford}
\def\Michigantext{University of Michigan}
\affil{Michigan}
\def\Ubctext{University of British Columbia, Canada}
\affil{Ubc}
\def\Bouldertext{University of Colorado Boulder}
\affil{Boulder}
\def\Minnesotatext{University of Minnesota}
\affil{Minnesota}
\def\Laltext{Laboratoire de l'Accélérateur Linéaire, France}
\affil{Lal}
\def\Columbiatext{Columbia University}
\affil{Columbia}
\def\Osutext{The Ohio State University}
\affil{Osu}
\def\Torontotext{University of Toronto, Canada}
\affil{Toronto}
\def\Fsutext{Florida State University}
\affil{Fsu}
\def\Davistext{University of California, Davis}
\affil{Davis}
\def\Pitttext{University of Pittsburgh}
\affil{Pitt}
\def\Ferraratext{Università di Ferrara, Italy}
\affil{Ferrara}
\def\Sussextext{University of Sussex, United Kingdom}
\affil{Sussex}
\def\Stonytext{Stony Brook University}
\affil{Stony}
\def\Madisontext{University of Wisconsin - Madison}
\affil{Madison}
\def\Santabarbaratext{University of California, Santa Barbara}
\affil{Santabarbara}
\def\Lpsctext{Laboratoire de Physique Subatomique & Cosmologie - Institut national de physique nucléaire et de physique des particules (Centre National de la Recherche Scientifique) / Université Grenoble Alpes}
\affil{Lpsc}
\def\Kingstext{King's College London, United Kingdom}
\affil{Kings}
\def\Asutext{Arizona State University}
\affil{Asu}
\def\Ceatext{Commissariat à l'Energie Atomique - Saclay, France}
\affil{Cea}
\def\Usctext{University of Southern California}
\affil{Usc}
\def\Bohrtext{Niels Bohr Institute, Denmark}
\affil{Bohr}
\def\Orsaytext{Institut d'Astrophysique Spatiale - Orsay, France}
\affil{Orsay}
\def\Sfutext{Simon Fraser University, Canada}
\affil{Sfu}
\def\Oslotext{University of Oslo, Norway}
\affil{Oslo}
\def\Melbournetext{University of Melbourne, Australia}
\affil{Melbourne}
\def\Casetext{Case Western Reserve University}
\affil{Case}
\def\Pennstatetext{The Pennsylvania State University}
\affil{Pennstate}
\def\Brookhaventext{Brookhaven National Laboratory}
\affil{Brookhaven}
\def\Swarthmoretext{Swarthmore College}
\affil{Swarthmore}
\def\Hpdtext{High Precision Devices, Boulder, CO}
\affil{Hpd}
\def\Umasstext{University of Massachusetts, Amherst}
\affil{Umass}
\def\Iucaatext{Inter-University Centre for Astronomy and Astrophysics, India}
\affil{Iucaa}
\def\Saotext{Smithsonian Astrophysical Observatory}
\affil{Sao}
\def\Mittext{Massachusetts Institute of Technology}
\affil{Mit}
\def\Browntext{Brown University}
\affil{Brown}
\def\Syracusetext{Syracuse University}
\affil{Syracuse}
\def\Gsfctext{National Aeronautics and Space Administration Goddard Space Flight Center}
\affil{Gsfc}

\begin{center}
\textbf{List of Endorsers}
\end{center}

The following people have endorsed the science case for CMB-S4 as presented here and many of them have contributed directly to the writing of this document:

Kevork N.~Abazajian\textsuperscript{\ref{Irvine}},
Peter Adshead\textsuperscript{\ref{Ill}},
James Aguirre\textsuperscript{\ref{Penn}},
Zeeshan Ahmed\textsuperscript{\ref{Slac}},
Simone Aiola\textsuperscript{\ref{Princeton}},
Yacine Ali-Haimoud\textsuperscript{\ref{Hopkins}},
Steven W.~Allen\textsuperscript{\ref{Stanford}},
David Alonso\textsuperscript{\ref{Oxford}},
Adam Anderson\textsuperscript{\ref{Fermi}},
James Annis\textsuperscript{\ref{Fermi}},
John W.~Appel\textsuperscript{\ref{Hopkins}}, 
Douglas E.~Applegate\textsuperscript{\ref{Chicago}}, 
Kam S.~Arnold\textsuperscript{\ref{Sandiego}}, 
Jason E.~Austermann\textsuperscript{\ref{Nist}},
Carlo Baccigalupi\textsuperscript{\ref{Sissa}}, 
Darcy Barron\textsuperscript{\ref{Berkeley}}, 
James G.~Bartlett\textsuperscript{\ref{Apc}}, 
Ritoban Basu Thakur\textsuperscript{\ref{Chicago}},
Nicholas Battaglia\textsuperscript{\ref{Princeton}},
Daniel Baumann\textsuperscript{\ref{Cambridge}},
Karim Benabed\textsuperscript{\ref{Iap}}, 
Amy N.~Bender\textsuperscript{\ref{Anl}}, 
Charles L.~Bennett\textsuperscript{\ref{Hopkins}},
Bradford A.~Benson\textsuperscript{\ref{Fermi}},
Colin A.~Bischoff\textsuperscript{\ref{Cincy}},
Lindsey Bleem\textsuperscript{\ref{Anl}}, 
J.~Richard Bond\textsuperscript{\ref{Cita}}, 
Julian Borrill\textsuperscript{\ref{Lbnl}}, 
François R.~Bouchet\textsuperscript{\ref{Iap}}, 
Michael L.~Brown\textsuperscript{\ref{Manchester}},
Christopher Brust\textsuperscript{\ref{Perimeter}}, 
Victor Buza\textsuperscript{\ref{Harvard}}, 
Karen Byrum\textsuperscript{\ref{Anl}}, 
Giovanni Cabass\textsuperscript{\ref{Sapienza}}, 
Erminia Calabrese\textsuperscript{\ref{Oxford}}, 
Robert Caldwell\textsuperscript{\ref{Dartmouth}}, 
John E.~Carlstrom\textsuperscript{\ref{Chicago}}, 
Anthony Challinor\textsuperscript{\ref{Cambridge}}, 
Clarence L.~Chang\textsuperscript{\ref{Anl}}, 
Hsin C.~Chiang\textsuperscript{\ref{Kwazulu}},
David T.~Chuss\textsuperscript{\ref{Nova}},
Asantha Cooray\textsuperscript{\ref{Irvine}}, 
Nicholas F.~Cothard\textsuperscript{\ref{Cornell}}, 
Thomas M.~Crawford\textsuperscript{\ref{Chicago}}, 
Brendan Crill\textsuperscript{\ref{Jpl}},
Abigail Crites\textsuperscript{\ref{Caltech}},
Francis-Yan Cyr-Racine\textsuperscript{\ref{Harvard}},
Francesco de Bernardis\textsuperscript{\ref{Cornell}}, 
Paolo M.~de Bernardis\textsuperscript{\ref{Sapienza}},
Tijmen de Haan\textsuperscript{\ref{Berkeley}},
Jacques Delabrouille\textsuperscript{\ref{Cnrs}}, 
Marcel Demarteau\textsuperscript{\ref{Anl}},
Mark Devlin\textsuperscript{\ref{Penn}}, 
Sperello di Serego Alighieri\textsuperscript{\ref{Arcetri}}, 
Eleonora di Valentino\textsuperscript{\ref{Iap}},
Clive Dickinson\textsuperscript{\ref{Manchester}},
Matt Dobbs\textsuperscript{\ref{Mcgill}},
Scott Dodelson\textsuperscript{\ref{Fermi}}, 
Olivier Dore\textsuperscript{\ref{Jpl}},
Joanna Dunkley\textsuperscript{\ref{Princeton}},
Cora Dvorkin\textsuperscript{\ref{Harvard}},
Josquin Errard\textsuperscript{\ref{Ilp}},
Thomas Essinger-Hileman\textsuperscript{\ref{Hopkins}},
Giulio Fabbian\textsuperscript{\ref{Sissa}},
Stephen Feeney\textsuperscript{\ref{Cca}},
Simone Ferraro\textsuperscript{\ref{Berkeley}}, 
Jeffrey P.~Filippini\textsuperscript{\ref{Ill}},
Raphael Flauger\textsuperscript{\ref{Sandiego}}, 
Aurelien A.~Fraisse\textsuperscript{\ref{Princeton}},
George M.~Fuller\textsuperscript{\ref{Sandiego}},
Patricio A.~Gallardo\textsuperscript{\ref{Cornell}},
Silvia Galli\textsuperscript{\ref{Iap}},
Jason Gallicchio\textsuperscript{\ref{Mudd}},
Ken Ganga\textsuperscript{\ref{Apc}},
Enrique Gaztanaga\textsuperscript{\ref{Ice}},
Martina Gerbino\textsuperscript{\ref{Stockholm}},
Mandeep S.~S.~Gill\textsuperscript{\ref{Stanford}},
Yannick Giraud-Héraud\textsuperscript{\ref{Apc}},
Vera Gluscevic\textsuperscript{\ref{Ias}},
Sunil Golwala\textsuperscript{\ref{Caltech}},
Krzysztof M.~Gorski\textsuperscript{\ref{Jpl}},
Daniel Green\textsuperscript{\ref{Berkeley}},
Daniel Grin\textsuperscript{\ref{Haverford}},
Evan Grohs\textsuperscript{\ref{Michigan}},
Riccardo Gualtieri\textsuperscript{\ref{Ill}}, 
Jon E.~Gudmundsson\textsuperscript{\ref{Stockholm}},
Grantland Hall\textsuperscript{\ref{Harvard}},
Mark Halpern\textsuperscript{\ref{Ubc}},
Nils W.~Halverson\textsuperscript{\ref{Boulder}},
Shaul Hanany\textsuperscript{\ref{Minnesota}},
Shawn Henderson\textsuperscript{\ref{Cornell}},
Jason W.~Henning\textsuperscript{\ref{Chicago}},
Sophie Henrot-Versille\textsuperscript{\ref{Lal}},
Sergi R.~Hildebrandt\textsuperscript{\ref{Caltech}},
J. Colin Hill\textsuperscript{\ref{Columbia}},
Christopher M.~Hirata\textsuperscript{\ref{Osu}},
Eric Hivon\textsuperscript{\ref{Iap}},
Ren\'{e}e Hlo\v{z}ek\textsuperscript{\ref{Toronto}},
Gilbert Holder\textsuperscript{\ref{Ill}},
William Holzapfel\textsuperscript{\ref{Berkeley}},
Wayne Hu\textsuperscript{\ref{Chicago}},
Johannes Hubmayr\textsuperscript{\ref{Nist}},
Kevin M.~Huffenberger\textsuperscript{\ref{Fsu}},
Kent Irwin\textsuperscript{\ref{Stanford}},
Bradley R.~Johnson\textsuperscript{\ref{Columbia}}, 
William C.~Jones\textsuperscript{\ref{Princeton}},
Marc Kamionkowski\textsuperscript{\ref{Hopkins}},
Brian Keating\textsuperscript{\ref{Sandiego}},
Sarah Kernasovskiy\textsuperscript{\ref{Stanford}},
Reijo Keskitalo\textsuperscript{\ref{Lbnl}},
Theodore Kisner\textsuperscript{\ref{Lbnl}},
Lloyd Knox\textsuperscript{\ref{Davis}},
Brian J.~Koopman\textsuperscript{\ref{Cornell}},
Arthur Kosowsky\textsuperscript{\ref{Pitt}},
John Kovac\textsuperscript{\ref{Harvard}},
Ely D.~Kovetz\textsuperscript{\ref{Hopkins}},
Nicoletta Krachmalnicoff\textsuperscript{\ref{Sissa}},
Chao-Lin Kuo\textsuperscript{\ref{Slac}},
Akito Kusaka\textsuperscript{\ref{Berkeley}},
Nicole A.~Larsen\textsuperscript{\ref{Chicago}},
Massimiliano Lattanzi\textsuperscript{\ref{Ferrara}},
Charles R.~Lawrence\textsuperscript{\ref{Jpl}},
Maude Le Jeune\textsuperscript{\ref{Apc}},
Adrian T.~Lee\textsuperscript{\ref{Berkeley}},
Antony Lewis\textsuperscript{\ref{Sussex}},
Marc Lilley\textsuperscript{\ref{Iap}},
Thibaut Louis\textsuperscript{\ref{Iap}},
Marilena Loverde\textsuperscript{\ref{Stony}},
Amy Lowitz\textsuperscript{\ref{Madison}},
Philip M.~Lubin\textsuperscript{\ref{Santabarbara}},
Juan J.~F.~Macias-Perez\textsuperscript{\ref{Lpsc}},
Mathew S.~Madhavacheril\textsuperscript{\ref{Princeton}},
Adam Mantz\textsuperscript{\ref{Stanford}},
David J.~E.~Marsh\textsuperscript{\ref{Kings}},
Silvia R.~M.~Masi\textsuperscript{\ref{Sapienza}},
Philip Mauskopf\textsuperscript{\ref{Asu}},
Jeffrey McMahon\textsuperscript{\ref{Michigan}},
Pieter Daniel Meerburg\textsuperscript{\ref{Cita}},
Alessandro Melchiorri\textsuperscript{\ref{Sapienza}},
Jean-Baptiste Melin\textsuperscript{\ref{Cea}},
Stephan Meyer\textsuperscript{\ref{Chicago}},
Joel Meyers\textsuperscript{\ref{Cita}},
Amber D.~Miller\textsuperscript{\ref{Usc}},
Laura M.~Mocanu\textsuperscript{\ref{Chicago}},
Lorenzo Moncelsi\textsuperscript{\ref{Caltech}},
Julian B.~Munoz\textsuperscript{\ref{Hopkins}},
Andrew Nadolski\textsuperscript{\ref{Ill}},
Pavel Naselsky\textsuperscript{\ref{Bohr}},
Paolo Natoli\textsuperscript{\ref{Ferrara}},
Ho Nam Nguyen\textsuperscript{\ref{Stony}},
Michael D.~Niemack\textsuperscript{\ref{Cornell}},
Stephen Padin\textsuperscript{\ref{Chicago}},
Luca Pagano\textsuperscript{\ref{Orsay}},
Lyman Page\textsuperscript{\ref{Princeton}},
Robert Bruce Partridge\textsuperscript{\ref{Haverford}},
Guillaume Patanchon\textsuperscript{\ref{Apc}},
Timothy J.~Pearson\textsuperscript{\ref{Caltech}},
Marco Peloso\textsuperscript{\ref{Minnesota}},
Julien Peloton\textsuperscript{\ref{Sussex}},
Olivier Perdereau\textsuperscript{\ref{Lal}},
Laurence Perotto\textsuperscript{\ref{Lpsc}},
Francesco Piacentini\textsuperscript{\ref{Sapienza}},
Michel Piat\textsuperscript{\ref{Apc}},
Levon Pogosian\textsuperscript{\ref{Sfu}},
Clement Pryke\textsuperscript{\ref{Minnesota}},
Benjamin Racine\textsuperscript{\ref{Oslo}},
Srinivasan Raghunathan\textsuperscript{\ref{Melbourne}},
Alexandra Rahlin\textsuperscript{\ref{Fermi}},
Marco Raveri\textsuperscript{\ref{Chicago}},
Christian L.~Reichardt\textsuperscript{\ref{Melbourne}},
Mathieu Remazeilles\textsuperscript{\ref{Manchester}},
Graca Rocha\textsuperscript{\ref{Jpl}},
Natalie A.~Roe\textsuperscript{\ref{Lbnl}},
Aditya Rotti\textsuperscript{\ref{Fsu}},
John Ruhl\textsuperscript{\ref{Case}},
Laura Salvati\textsuperscript{\ref{Sapienza}},
Emmanuel Schaan\textsuperscript{\ref{Princeton}},
Marcel M.~Schmittfull\textsuperscript{\ref{Berkeley}},
Douglas Scott\textsuperscript{\ref{Ubc}},
Neelima Sehgal\textsuperscript{\ref{Stony}},
Sarah Shandera\textsuperscript{\ref{Pennstate}},
Christopher Sheehy\textsuperscript{\ref{Brookhaven}},
Blake D. Sherwin\textsuperscript{\ref{Berkeley}},
Erik Shirokoff\textsuperscript{\ref{Chicago}},
Eva Silverstein\textsuperscript{\ref{Stanford}},
Sara M.~Simon\textsuperscript{\ref{Michigan}},
Tristan L.~Smith\textsuperscript{\ref{Swarthmore}},
Michael Snow\textsuperscript{\ref{Hpd}},
Lorenzo Sorbo\textsuperscript{\ref{Umass}},
Tarun Souradeep\textsuperscript{\ref{Iucaa}},
Suzanne T.~Staggs\textsuperscript{\ref{Princeton}},
Antony A.~Stark\textsuperscript{\ref{Sao}},
Glenn D.~Starkman\textsuperscript{\ref{Case}},
George F.~Stein\textsuperscript{\ref{Cita}},
Jason R.~Stevens\textsuperscript{\ref{Cornell}},
Radek Stompor\textsuperscript{\ref{Apc}},
Kyle T.~Story\textsuperscript{\ref{Stanford}},
Chris Stoughton\textsuperscript{\ref{Fermi}},
Meng Su\textsuperscript{\ref{Mit}},
Aritoki Suzuki\textsuperscript{\ref{Berkeley}},
Grant P.~Teply\textsuperscript{\ref{Sandiego}},
Peter Timbie\textsuperscript{\ref{Madison}},
Jesse I.~Treu\textsuperscript{\ref{Princeton}},
Matthieu Tristram\textsuperscript{\ref{Lal}},
Gregory Tucker\textsuperscript{\ref{Brown}},
Sunny Vagnozzi\textsuperscript{\ref{Stockholm}},
Alexander van Engelen\textsuperscript{\ref{Cita}},
Eve M.~Vavagiakis\textsuperscript{\ref{Cornell}},
Joaquin D.~Vieira\textsuperscript{\ref{Ill}},
Abigail G.~Vieregg\textsuperscript{\ref{Chicago}}, 
Sebastian von Hausegger\textsuperscript{\ref{Bohr}},
Benjamin D.~Wandelt\textsuperscript{\ref{Iap}},
Scott Watson\textsuperscript{\ref{Syracuse}},
Nathan Whitehorn\textsuperscript{\ref{Berkeley}},
Edward J.~Wollack\textsuperscript{\ref{Gsfc}},
W.~L.~Kimmy Wu\textsuperscript{\ref{Berkeley}},
Zhilei Xu\textsuperscript{\ref{Hopkins}},
Ki Won Yoon\textsuperscript{\ref{Slac}},
Matias Zaldarriaga\textsuperscript{\ref{Ias}}.

\noindent
\textsuperscript{\ref{Irvine}}\Irvinetext

\noindent
\textsuperscript{\ref{Ill}}\Illtext

\noindent
\textsuperscript{\ref{Penn}}\Penntext

\noindent
\textsuperscript{\ref{Slac}}

\noindent
\textsuperscript{\ref{Princeton}}

\noindent
\textsuperscript{\ref{Hopkins}}

\noindent
\textsuperscript{\ref{Stanford}}

\noindent
\textsuperscript{\ref{Oxford}}

\noindent
\textsuperscript{\ref{Fermi}}

\noindent
\textsuperscript{\ref{Chicago}}

\noindent
\textsuperscript{\ref{Sandiego}}

\noindent
\textsuperscript{\ref{Nist}}

\noindent
\textsuperscript{\ref{Sissa}}

\noindent
\textsuperscript{\ref{Berkeley}}

\noindent
\textsuperscript{\ref{Apc}}

\noindent
\textsuperscript{\ref{Iap}}

\noindent
\textsuperscript{\ref{Anl}}

\noindent
\textsuperscript{\ref{Cincy}}

\noindent
\textsuperscript{\ref{Cita}}

\noindent
\textsuperscript{\ref{Lbnl}}

\noindent
\textsuperscript{\ref{Manchester}}

\noindent
\textsuperscript{\ref{Perimeter}}

\noindent
\textsuperscript{\ref{Harvard}}

\noindent
\textsuperscript{\ref{Sapienza}}

\noindent
\textsuperscript{\ref{Dartmouth}}

\noindent
\textsuperscript{\ref{Kwazulu}}

\noindent
\textsuperscript{\ref{Nova}}

\noindent
\textsuperscript{\ref{Cornell}}

\noindent
\textsuperscript{\ref{Jpl}}

\noindent
\textsuperscript{\ref{Caltech}}

\noindent
\textsuperscript{\ref{Cnrs}}

\noindent
\textsuperscript{\ref{Arcetri}}

\noindent
\textsuperscript{\ref{Mcgill}}

\noindent
\textsuperscript{\ref{Ilp}}

\noindent
\textsuperscript{\ref{Cca}}

\noindent
\textsuperscript{\ref{Mudd}}

\noindent
\textsuperscript{\ref{Ice}}

\noindent
\textsuperscript{\ref{Stockholm}}

\noindent
\textsuperscript{\ref{Ias}}

\noindent
\textsuperscript{\ref{Haverford}}

\noindent
\textsuperscript{\ref{Michigan}}

\noindent
\textsuperscript{\ref{Ubc}}

\noindent
\textsuperscript{\ref{Boulder}}

\noindent
\textsuperscript{\ref{Minnesota}}

\noindent
\textsuperscript{\ref{Lal}}

\noindent
\textsuperscript{\ref{Columbia}}

\noindent
\textsuperscript{\ref{Osu}}

\noindent
\textsuperscript{\ref{Toronto}}

\noindent
\textsuperscript{\ref{Fsu}}

\noindent
\textsuperscript{\ref{Davis}}

\noindent
\textsuperscript{\ref{Pitt}}

\noindent
\textsuperscript{\ref{Ferrara}}

\noindent
\textsuperscript{\ref{Sussex}}

\noindent
\textsuperscript{\ref{Stony}}

\noindent
\textsuperscript{\ref{Madison}}

\noindent
\textsuperscript{\ref{Santabarbara}}

\noindent
\textsuperscript{\ref{Lpsc}}

\noindent
\textsuperscript{\ref{Kings}}

\noindent
\textsuperscript{\ref{Asu}}

\noindent
\textsuperscript{\ref{Cea}}

\noindent
\textsuperscript{\ref{Usc}}

\noindent
\textsuperscript{\ref{Bohr}}

\noindent
\textsuperscript{\ref{Orsay}}

\noindent
\textsuperscript{\ref{Sfu}}

\noindent
\textsuperscript{\ref{Oslo}}

\noindent
\textsuperscript{\ref{Melbourne}}

\noindent
\textsuperscript{\ref{Case}}

\noindent
\textsuperscript{\ref{Pennstate}}

\noindent
\textsuperscript{\ref{Brookhaven}}

\noindent
\textsuperscript{\ref{Swarthmore}}

\noindent
\textsuperscript{\ref{Hpd}}

\noindent
\textsuperscript{\ref{Umass}}

\noindent
\textsuperscript{\ref{Iucaa}}

\noindent
\textsuperscript{\ref{Sao}}

\noindent
\textsuperscript{\ref{Mit}}

\noindent
\textsuperscript{\ref{Brown}}

\noindent
\textsuperscript{\ref{Syracuse}}

\noindent
\textsuperscript{\ref{Gsfc}}




==> endorser_list_indexed_temp.tex <==
\newcounter{affilcount}

\newcommand{\affil}[1]{\refstepcounter{affilcount}\label{#1}}

\def\Irvinetext{University of California, Irvine}
\affil{Irvine}
\def\Illtext{University of Illinois, Urbana-Champaign}
\affil{Ill}
\def\Penntext{University of Pennsylvania}
\affil{Penn}
\def\Slactext{SLAC National Accelerator Laboratory}
\affil{Slac}
\def\Princetontext{Princeton University}
\affil{Princeton}
\def\Hopkinstext{Johns Hopkins University}
\affil{Hopkins}
\def\Stanfordtext{Stanford University}
\affil{Stanford}
\def\Oxfordtext{University of Oxford, United Kingdom}
\affil{Oxford}
\def\Fermitext{Fermilab National Accelerator Laboratory}
\affil{Fermi}
\def\Chicagotext{University of Chicago}
\affil{Chicago}
\def\Sandiegotext{University of California, San Diego}
\affil{Sandiego}
\def\Nisttext{National Institute of Standards and Technology}
\affil{Nist}
\def\Sissatext{Scuola Internazionale Superiore di Studi Avanzati, Trieste, Italy}
\affil{Sissa}
\def\Berkeleytext{University of California, Berkeley}
\affil{Berkeley}
\def\Apctext{Laboratoire AstroParticule et Cosmologie - Université Paris Diderot, France}
\affil{Apc}
\def\Cambridgetext{University of Cambridge, United Kingdom}
\affil{Cambridge}
\def\Iaptext{Institut d'Astrophysique de Paris - Université Pierre et Marie Curie /  Centre National de la Recherche Scientifique, France}
\affil{Iap}
\def\Anltext{Argonne National Laboratory}
\affil{Anl}
\def\Cincytext{University of Cincinnati}
\affil{Cincy}
\def\Citatext{Canadian Institute For Theoretical Astrophysics, Canada}
\affil{Cita}
\def\Lbnltext{Lawrence Berkeley National Laboratory}
\affil{Lbnl}
\def\Manchestertext{University of Manchester, United Kingdom}
\affil{Manchester}
\def\Perimetertext{Perimeter Institute, Canada}
\affil{Perimeter}
\def\Harvardtext{Harvard University}
\affil{Harvard}
\def\Sapienzatext{Sapienza - Università di Roma, Italy}
\affil{Sapienza}
\def\Dartmouthtext{Dartmouth College}
\affil{Dartmouth}
\def\Kwazulutext{University of KwaZulu-Natal, South Africa}
\affil{Kwazulu}
\def\Novatext{Villanova University}
\affil{Nova}
\def\Cornelltext{Cornell University}
\affil{Cornell}
\def\Jpltext{Jet Propulsion Laboratory}
\affil{Jpl}
\def\Caltechtext{California Institute of Technology}
\affil{Caltech}
\def\Cnrstext{Centre National de la Recherche Scientifique, France}
\affil{Cnrs}
\def\Arcetritext{Istituto Nazionale di Astrofisica - Osservatorio Astrofisico di Arcetri, Italy}
\affil{Arcetri}
\def\Mcgilltext{McGill University, Canada}
\affil{Mcgill}
\def\Ilptext{Institut Lagrange Paris - Université Pierre et Marie Curie /  Centre National de la Recherche Scientifique, France}
\affil{Ilp}
\def\Ccatext{Center for Computational Astrophysics}
\affil{Cca}
\def\Muddtext{Harvey Mudd College}
\affil{Mudd}
\def\Icetext{Institut de Ciències de l'Espai, Spain}
\affil{Ice}
\def\Stockholmtext{Stockholm University, Sweden}
\affil{Stockholm}
\def\Iastext{Institute for Advanced Study}
\affil{Ias}
\def\Haverfordtext{Haverford College}
\affil{Haverford}
\def\Michigantext{University of Michigan}
\affil{Michigan}
\def\Ubctext{University of British Columbia, Canada}
\affil{Ubc}
\def\Bouldertext{University of Colorado Boulder}
\affil{Boulder}
\def\Minnesotatext{University of Minnesota}
\affil{Minnesota}
\def\Laltext{Laboratoire de l'Accélérateur Linéaire, France}
\affil{Lal}
\def\Columbiatext{Columbia University}
\affil{Columbia}
\def\Osutext{The Ohio State University}
\affil{Osu}
\def\Torontotext{University of Toronto, Canada}
\affil{Toronto}
\def\Fsutext{Florida State University}
\affil{Fsu}
\def\Davistext{University of California, Davis}
\affil{Davis}
\def\Pitttext{University of Pittsburgh}
\affil{Pitt}
\def\Ferraratext{Università di Ferrara, Italy}
\affil{Ferrara}
\def\Sussextext{University of Sussex, United Kingdom}
\affil{Sussex}
\def\Stonytext{Stony Brook University}
\affil{Stony}
\def\Madisontext{University of Wisconsin - Madison}
\affil{Madison}
\def\Santabarbaratext{University of California, Santa Barbara}
\affil{Santabarbara}
\def\Lpsctext{Laboratoire de Physique Subatomique & Cosmologie - Institut national de physique nucléaire et de physique des particules (Centre National de la Recherche Scientifique) / Université Grenoble Alpes}
\affil{Lpsc}
\def\Kingstext{King's College London, United Kingdom}
\affil{Kings}
\def\Asutext{Arizona State University}
\affil{Asu}
\def\Ceatext{Commissariat à l'Energie Atomique - Saclay, France}
\affil{Cea}
\def\Usctext{University of Southern California}
\affil{Usc}
\def\Bohrtext{Niels Bohr Institute, Denmark}
\affil{Bohr}
\def\Orsaytext{Institut d'Astrophysique Spatiale - Orsay, France}
\affil{Orsay}
\def\Sfutext{Simon Fraser University, Canada}
\affil{Sfu}
\def\Oslotext{University of Oslo, Norway}
\affil{Oslo}
\def\Melbournetext{University of Melbourne, Australia}
\affil{Melbourne}
\def\Casetext{Case Western Reserve University}
\affil{Case}
\def\Pennstatetext{The Pennsylvania State University}
\affil{Pennstate}
\def\Brookhaventext{Brookhaven National Laboratory}
\affil{Brookhaven}
\def\Swarthmoretext{Swarthmore College}
\affil{Swarthmore}
\def\Hpdtext{High Precision Devices, Boulder, CO}
\affil{Hpd}
\def\Umasstext{University of Massachusetts, Amherst}
\affil{Umass}
\def\Iucaatext{Inter-University Centre for Astronomy and Astrophysics, India}
\affil{Iucaa}
\def\Saotext{Smithsonian Astrophysical Observatory}
\affil{Sao}
\def\Mittext{Massachusetts Institute of Technology}
\affil{Mit}
\def\Browntext{Brown University}
\affil{Brown}
\def\Syracusetext{Syracuse University}
\affil{Syracuse}
\def\Gsfctext{National Aeronautics and Space Administration Goddard Space Flight Center}
\affil{Gsfc}

\begin{center}
\textbf{List of Endorsers}
\end{center}

The following people have endorsed the science case for CMB-S4 as presented here and many of them have contributed directly to the writing of this document:

Kevork N.~Abazajian\textsuperscript{\ref{Irvine}},
Peter Adshead\textsuperscript{\ref{Ill}},
James Aguirre\textsuperscript{\ref{Penn}},
Zeeshan Ahmed\textsuperscript{\ref{Slac}},
Simone Aiola\textsuperscript{\ref{Princeton}},
Yacine Ali-Haimoud\textsuperscript{\ref{Hopkins}},
Steven W.~Allen\textsuperscript{\ref{Stanford}},
David Alonso\textsuperscript{\ref{Oxford}},
Adam Anderson\textsuperscript{\ref{Fermi}},
James Annis\textsuperscript{\ref{Fermi}},
John W.~Appel\textsuperscript{\ref{Hopkins}}, 
Douglas E.~Applegate\textsuperscript{\ref{Chicago}}, 
Kam S.~Arnold\textsuperscript{\ref{Sandiego}}, 
Jason E.~Austermann\textsuperscript{\ref{Nist}},
Carlo Baccigalupi\textsuperscript{\ref{Sissa}}, 
Darcy Barron\textsuperscript{\ref{Berkeley}}, 
James G.~Bartlett\textsuperscript{\ref{Apc}}, 
Ritoban Basu Thakur\textsuperscript{\ref{Chicago}},
Nicholas Battaglia\textsuperscript{\ref{Princeton}},
Daniel Baumann\textsuperscript{\ref{Cambridge}},
Karim Benabed\textsuperscript{\ref{Iap}}, 
Amy N.~Bender\textsuperscript{\ref{Anl}}, 
Charles L.~Bennett\textsuperscript{\ref{Hopkins}},
Bradford A.~Benson\textsuperscript{\ref{Fermi}},
Colin A.~Bischoff\textsuperscript{\ref{Cincy}},
Lindsey Bleem\textsuperscript{\ref{Anl}}, 
J.~Richard Bond\textsuperscript{\ref{Cita}}, 
Julian Borrill\textsuperscript{\ref{Lbnl}}, 
François R.~Bouchet\textsuperscript{\ref{Iap}}, 
Michael L.~Brown\textsuperscript{\ref{Manchester}},
Christopher Brust\textsuperscript{\ref{Perimeter}}, 
Victor Buza\textsuperscript{\ref{Harvard}}, 
Karen Byrum\textsuperscript{\ref{Anl}}, 
Giovanni Cabass\textsuperscript{\ref{Sapienza}}, 
Erminia Calabrese\textsuperscript{\ref{Oxford}}, 
Robert Caldwell\textsuperscript{\ref{Dartmouth}}, 
John E.~Carlstrom\textsuperscript{\ref{Chicago}}, 
Anthony Challinor\textsuperscript{\ref{Cambridge}}, 
Clarence L.~Chang\textsuperscript{\ref{Anl}}, 
Hsin C.~Chiang\textsuperscript{\ref{Kwazulu}},
David T.~Chuss\textsuperscript{\ref{Nova}},
Asantha Cooray\textsuperscript{\ref{Irvine}}, 
Nicholas F.~Cothard\textsuperscript{\ref{Cornell}}, 
Thomas M.~Crawford\textsuperscript{\ref{Chicago}}, 
Brendan Crill\textsuperscript{\ref{Jpl}},
Abigail Crites\textsuperscript{\ref{Caltech}},
Francis-Yan Cyr-Racine\textsuperscript{\ref{Harvard}},
Francesco de Bernardis\textsuperscript{\ref{Cornell}}, 
Paolo M.~de Bernardis\textsuperscript{\ref{Sapienza}},
Tijmen de Haan\textsuperscript{\ref{Berkeley}},
Jacques Delabrouille\textsuperscript{\ref{Cnrs}}, 
Marcel Demarteau\textsuperscript{\ref{Anl}},
Mark Devlin\textsuperscript{\ref{Penn}}, 
Sperello di Serego Alighieri\textsuperscript{\ref{Arcetri}}, 
Eleonora di Valentino\textsuperscript{\ref{Iap}},
Clive Dickinson\textsuperscript{\ref{Manchester}},
Matt Dobbs\textsuperscript{\ref{Mcgill}},
Scott Dodelson\textsuperscript{\ref{Fermi}}, 
Olivier Dore\textsuperscript{\ref{Jpl}},
Joanna Dunkley\textsuperscript{\ref{Princeton}},
Cora Dvorkin\textsuperscript{\ref{Harvard}},
Josquin Errard\textsuperscript{\ref{Ilp}},
Thomas Essinger-Hileman\textsuperscript{\ref{Hopkins}},
Giulio Fabbian\textsuperscript{\ref{Sissa}},
Stephen Feeney\textsuperscript{\ref{Cca}},
Simone Ferraro\textsuperscript{\ref{Berkeley}}, 
Jeffrey P.~Filippini\textsuperscript{\ref{Ill}},
Raphael Flauger\textsuperscript{\ref{Sandiego}}, 
Aurelien A.~Fraisse\textsuperscript{\ref{Princeton}},
George M.~Fuller\textsuperscript{\ref{Sandiego}},
Patricio A.~Gallardo\textsuperscript{\ref{Cornell}},
Silvia Galli\textsuperscript{\ref{Iap}},
Jason Gallicchio\textsuperscript{\ref{Mudd}},
Ken Ganga\textsuperscript{\ref{Apc}},
Enrique Gaztanaga\textsuperscript{\ref{Ice}},
Martina Gerbino\textsuperscript{\ref{Stockholm}},
Mandeep S.~S.~Gill\textsuperscript{\ref{Stanford}},
Yannick Giraud-Héraud\textsuperscript{\ref{Apc}},
Vera Gluscevic\textsuperscript{\ref{Ias}},
Sunil Golwala\textsuperscript{\ref{Caltech}},
Krzysztof M.~Gorski\textsuperscript{\ref{Jpl}},
Daniel Green\textsuperscript{\ref{Berkeley}},
Daniel Grin\textsuperscript{\ref{Haverford}},
Evan Grohs\textsuperscript{\ref{Michigan}},
Riccardo Gualtieri\textsuperscript{\ref{Ill}}, 
Jon E.~Gudmundsson\textsuperscript{\ref{Stockholm}},
Grantland Hall\textsuperscript{\ref{Harvard}},
Mark Halpern\textsuperscript{\ref{Ubc}},
Nils W.~Halverson\textsuperscript{\ref{Boulder}},
Shaul Hanany\textsuperscript{\ref{Minnesota}},
Shawn Henderson\textsuperscript{\ref{Cornell}},
Jason W.~Henning\textsuperscript{\ref{Chicago}},
Sophie Henrot-Versille\textsuperscript{\ref{Lal}},
Sergi R.~Hildebrandt\textsuperscript{\ref{Caltech}},
J. Colin Hill\textsuperscript{\ref{Columbia}},
Christopher M.~Hirata\textsuperscript{\ref{Osu}},
Eric Hivon\textsuperscript{\ref{Iap}},
Ren\'{e}e Hlo\v{z}ek\textsuperscript{\ref{Toronto}},
Gilbert Holder\textsuperscript{\ref{Ill}},
William Holzapfel\textsuperscript{\ref{Berkeley}},
Wayne Hu\textsuperscript{\ref{Chicago}},
Johannes Hubmayr\textsuperscript{\ref{Nist}},
Kevin M.~Huffenberger\textsuperscript{\ref{Fsu}},
Kent Irwin\textsuperscript{\ref{Stanford}},
Bradley R.~Johnson\textsuperscript{\ref{Columbia}}, 
William C.~Jones\textsuperscript{\ref{Princeton}},
Marc Kamionkowski\textsuperscript{\ref{Hopkins}},
Brian Keating\textsuperscript{\ref{Sandiego}},
Sarah Kernasovskiy\textsuperscript{\ref{Stanford}},
Reijo Keskitalo\textsuperscript{\ref{Lbnl}},
Theodore Kisner\textsuperscript{\ref{Lbnl}},
Lloyd Knox\textsuperscript{\ref{Davis}},
Brian J.~Koopman\textsuperscript{\ref{Cornell}},
Arthur Kosowsky\textsuperscript{\ref{Pitt}},
John Kovac\textsuperscript{\ref{Harvard}},
Ely D.~Kovetz\textsuperscript{\ref{Hopkins}},
Nicoletta Krachmalnicoff\textsuperscript{\ref{Sissa}},
Chao-Lin Kuo\textsuperscript{\ref{Slac}},
Akito Kusaka\textsuperscript{\ref{Berkeley}},
Nicole A.~Larsen\textsuperscript{\ref{Chicago}},
Massimiliano Lattanzi\textsuperscript{\ref{Ferrara}},
Charles R.~Lawrence\textsuperscript{\ref{Jpl}},
Maude Le Jeune\textsuperscript{\ref{Apc}},
Adrian T.~Lee\textsuperscript{\ref{Berkeley}},
Antony Lewis\textsuperscript{\ref{Sussex}},
Marc Lilley\textsuperscript{\ref{Iap}},
Thibaut Louis\textsuperscript{\ref{Iap}},
Marilena Loverde\textsuperscript{\ref{Stony}},
Amy Lowitz\textsuperscript{\ref{Madison}},
Philip M.~Lubin\textsuperscript{\ref{Santabarbara}},
Juan J.~F.~Macias-Perez\textsuperscript{\ref{Lpsc}},
Mathew S.~Madhavacheril\textsuperscript{\ref{Princeton}},
Adam Mantz\textsuperscript{\ref{Stanford}},
David J.~E.~Marsh\textsuperscript{\ref{Kings}},
Silvia R.~M.~Masi\textsuperscript{\ref{Sapienza}},
Philip Mauskopf\textsuperscript{\ref{Asu}},
Jeffrey McMahon\textsuperscript{\ref{Michigan}},
Pieter Daniel Meerburg\textsuperscript{\ref{Cita}},
Alessandro Melchiorri\textsuperscript{\ref{Sapienza}},
Jean-Baptiste Melin\textsuperscript{\ref{Cea}},
Stephan Meyer\textsuperscript{\ref{Chicago}},
Joel Meyers\textsuperscript{\ref{Cita}},
Amber D.~Miller\textsuperscript{\ref{Usc}},
Laura M.~Mocanu\textsuperscript{\ref{Chicago}},
Lorenzo Moncelsi\textsuperscript{\ref{Caltech}},
Julian B.~Munoz\textsuperscript{\ref{Hopkins}},
Andrew Nadolski\textsuperscript{\ref{Ill}},
Pavel Naselsky\textsuperscript{\ref{Bohr}},
Paolo Natoli\textsuperscript{\ref{Ferrara}},
Ho Nam Nguyen\textsuperscript{\ref{Stony}},
Michael D.~Niemack\textsuperscript{\ref{Cornell}},
Stephen Padin\textsuperscript{\ref{Chicago}},
Luca Pagano\textsuperscript{\ref{Orsay}},
Lyman Page\textsuperscript{\ref{Princeton}},
Robert Bruce Partridge\textsuperscript{\ref{Haverford}},
Guillaume Patanchon\textsuperscript{\ref{Apc}},
Timothy J.~Pearson\textsuperscript{\ref{Caltech}},
Marco Peloso\textsuperscript{\ref{Minnesota}},
Julien Peloton\textsuperscript{\ref{Sussex}},
Olivier Perdereau\textsuperscript{\ref{Lal}},
Laurence Perotto\textsuperscript{\ref{Lpsc}},
Francesco Piacentini\textsuperscript{\ref{Sapienza}},
Michel Piat\textsuperscript{\ref{Apc}},
Levon Pogosian\textsuperscript{\ref{Sfu}},
Clement Pryke\textsuperscript{\ref{Minnesota}},
Benjamin Racine\textsuperscript{\ref{Oslo}},
Srinivasan Raghunathan\textsuperscript{\ref{Melbourne}},
Alexandra Rahlin\textsuperscript{\ref{Fermi}},
Marco Raveri\textsuperscript{\ref{Chicago}},
Christian L.~Reichardt\textsuperscript{\ref{Melbourne}},
Mathieu Remazeilles\textsuperscript{\ref{Manchester}},
Graca Rocha\textsuperscript{\ref{Jpl}},
Natalie A.~Roe\textsuperscript{\ref{Lbnl}},
Aditya Rotti\textsuperscript{\ref{Fsu}},
John Ruhl\textsuperscript{\ref{Case}},
Laura Salvati\textsuperscript{\ref{Sapienza}},
Emmanuel Schaan\textsuperscript{\ref{Princeton}},
Marcel M.~Schmittfull\textsuperscript{\ref{Berkeley}},
Douglas Scott\textsuperscript{\ref{Ubc}},
Neelima Sehgal\textsuperscript{\ref{Stony}},
Sarah Shandera\textsuperscript{\ref{Pennstate}},
Christopher Sheehy\textsuperscript{\ref{Brookhaven}},
Blake D. Sherwin\textsuperscript{\ref{Berkeley}},
Erik Shirokoff\textsuperscript{\ref{Chicago}},
Eva Silverstein\textsuperscript{\ref{Stanford}},
Sara M.~Simon\textsuperscript{\ref{Michigan}},
Tristan L.~Smith\textsuperscript{\ref{Swarthmore}},
Michael Snow\textsuperscript{\ref{Hpd}},
Lorenzo Sorbo\textsuperscript{\ref{Umass}},
Tarun Souradeep\textsuperscript{\ref{Iucaa}},
Suzanne T.~Staggs\textsuperscript{\ref{Princeton}},
Antony A.~Stark\textsuperscript{\ref{Sao}},
Glenn D.~Starkman\textsuperscript{\ref{Case}},
George F.~Stein\textsuperscript{\ref{Cita}},
Jason R.~Stevens\textsuperscript{\ref{Cornell}},
Radek Stompor\textsuperscript{\ref{Apc}},
Kyle T.~Story\textsuperscript{\ref{Stanford}},
Chris Stoughton\textsuperscript{\ref{Fermi}},
Meng Su\textsuperscript{\ref{Mit}},
Aritoki Suzuki\textsuperscript{\ref{Berkeley}},
Grant P.~Teply\textsuperscript{\ref{Sandiego}},
Peter Timbie\textsuperscript{\ref{Madison}},
Jesse I.~Treu\textsuperscript{\ref{Princeton}},
Matthieu Tristram\textsuperscript{\ref{Lal}},
Gregory Tucker\textsuperscript{\ref{Brown}},
Sunny Vagnozzi\textsuperscript{\ref{Stockholm}},
Alexander van Engelen\textsuperscript{\ref{Cita}},
Eve M.~Vavagiakis\textsuperscript{\ref{Cornell}},
Joaquin D.~Vieira\textsuperscript{\ref{Ill}},
Abigail G.~Vieregg\textsuperscript{\ref{Chicago}}, 
Sebastian von Hausegger\textsuperscript{\ref{Bohr}},
Benjamin D.~Wandelt\textsuperscript{\ref{Iap}},
Scott Watson\textsuperscript{\ref{Syracuse}},
Nathan Whitehorn\textsuperscript{\ref{Berkeley}},
Edward J.~Wollack\textsuperscript{\ref{Gsfc}},
W.~L.~Kimmy Wu\textsuperscript{\ref{Berkeley}},
Zhilei Xu\textsuperscript{\ref{Hopkins}},
Ki Won Yoon\textsuperscript{\ref{Slac}},
Matias Zaldarriaga\textsuperscript{\ref{Ias}}.

\noindent
\textsuperscript{\ref{Irvine}}\Irvinetext

\noindent
\textsuperscript{\ref{Ill}}\Illtext

\noindent
\textsuperscript{\ref{Penn}}\Penntext

\noindent
\textsuperscript{\ref{Slac}}\Slactext

\noindent
\textsuperscript{\ref{Princeton}}\Princetontext

\noindent
\textsuperscript{\ref{Hopkins}}\Hopkinstext

\noindent
\textsuperscript{\ref{Stanford}}\Stanfordtext

\noindent
\textsuperscript{\ref{Oxford}}\Oxfordtext

\noindent
\textsuperscript{\ref{Fermi}}\Fermitext

\noindent
\textsuperscript{\ref{Chicago}}\Chicagotext

\noindent
\textsuperscript{\ref{Sandiego}}\Sandiegotext

\noindent
\textsuperscript{\ref{Nist}}\Nisttext

\noindent
\textsuperscript{\ref{Sissa}}\Sissatext

\noindent
\textsuperscript{\ref{Berkeley}}\Berkeleytext

\noindent
\textsuperscript{\ref{Apc}}\Apctext

\noindent
\textsuperscript{\ref{Iap}}\Iaptext

\noindent
\textsuperscript{\ref{Anl}}\Anltext

\noindent
\textsuperscript{\ref{Cincy}}\Cincytext

\noindent
\textsuperscript{\ref{Cita}}\Citatext

\noindent
\textsuperscript{\ref{Lbnl}}\Lbnltext

\noindent
\textsuperscript{\ref{Manchester}}\Manchestertext

\noindent
\textsuperscript{\ref{Perimeter}}\Perimetertext

\noindent
\textsuperscript{\ref{Harvard}}\Harvardtext

\noindent
\textsuperscript{\ref{Sapienza}}\Sapienzatext

\noindent
\textsuperscript{\ref{Dartmouth}}\Dartmouthtext

\noindent
\textsuperscript{\ref{Kwazulu}}\Kwazulutext

\noindent
\textsuperscript{\ref{Nova}}\Novatext

\noindent
\textsuperscript{\ref{Cornell}}\Cornelltext

\noindent
\textsuperscript{\ref{Jpl}}\Jpltext

\noindent
\textsuperscript{\ref{Caltech}}\Caltechtext

\noindent
\textsuperscript{\ref{Cnrs}}\Cnrstext

\noindent
\textsuperscript{\ref{Arcetri}}\Arcetritext

\noindent
\textsuperscript{\ref{Mcgill}}\Mcgilltext

\noindent
\textsuperscript{\ref{Ilp}}\Ilptext

\noindent
\textsuperscript{\ref{Cca}}\Ccatext

\noindent
\textsuperscript{\ref{Mudd}}\Muddtext

\noindent
\textsuperscript{\ref{Ice}}\Icetext

\noindent
\textsuperscript{\ref{Stockholm}}\Stockholmtext

\noindent
\textsuperscript{\ref{Ias}}\Iastext

\noindent
\textsuperscript{\ref{Haverford}}\Haverfordtext

\noindent
\textsuperscript{\ref{Michigan}}\Michigantext

\noindent
\textsuperscript{\ref{Ubc}}\Ubctext

\noindent
\textsuperscript{\ref{Boulder}}\Bouldertext

\noindent
\textsuperscript{\ref{Minnesota}}\Minnesotatext

\noindent
\textsuperscript{\ref{Lal}}\Laltext

\noindent
\textsuperscript{\ref{Columbia}}\Columbiatext

\noindent
\textsuperscript{\ref{Osu}}\Osutext

\noindent
\textsuperscript{\ref{Toronto}}\Torontotext

\noindent
\textsuperscript{\ref{Fsu}}\Fsutext

\noindent
\textsuperscript{\ref{Davis}}\Davistext

\noindent
\textsuperscript{\ref{Pitt}}\Pitttext

\noindent
\textsuperscript{\ref{Ferrara}}\Ferraratext

\noindent
\textsuperscript{\ref{Sussex}}\Sussextext

\noindent
\textsuperscript{\ref{Stony}}\Stonytext

\noindent
\textsuperscript{\ref{Madison}}\Madisontext

\noindent
\textsuperscript{\ref{Santabarbara}}\Santabarbaratext

\noindent
\textsuperscript{\ref{Lpsc}}\Lpsctext

\noindent
\textsuperscript{\ref{Kings}}\Kingstext

\noindent
\textsuperscript{\ref{Asu}}\Asutext

\noindent
\textsuperscript{\ref{Cea}}\Ceatext

\noindent
\textsuperscript{\ref{Usc}}\Usctext

\noindent
\textsuperscript{\ref{Bohr}}\Bohrtext

\noindent
\textsuperscript{\ref{Orsay}}\Orsaytext

\noindent
\textsuperscript{\ref{Sfu}}\Sfutext

\noindent
\textsuperscript{\ref{Oslo}}\Oslotext

\noindent
\textsuperscript{\ref{Melbourne}}\Melbournetext

\noindent
\textsuperscript{\ref{Case}}\Casetext

\noindent
\textsuperscript{\ref{Pennstate}}\Pennstatetext

\noindent
\textsuperscript{\ref{Brookhaven}}\Brookhaventext

\noindent
\textsuperscript{\ref{Swarthmore}}\Swarthmoretext

\noindent
\textsuperscript{\ref{Hpd}}\Hpdtext

\noindent
\textsuperscript{\ref{Umass}}\Umasstext

\noindent
\textsuperscript{\ref{Iucaa}}\Iucaatext

\noindent
\textsuperscript{\ref{Sao}}\Saotext

\noindent
\textsuperscript{\ref{Mit}}\Mittext

\noindent
\textsuperscript{\ref{Brown}}\Browntext

\noindent
\textsuperscript{\ref{Syracuse}}\Syracusetext

\noindent
\textsuperscript{\ref{Gsfc}}\Gsfctext




==> endorser_list_intermediate.tex <==
\begin{center}
\textbf{List of Endorsers}
\end{center}

The following people have endorsed the science case for CMB-S4 as presented here and many of them have contributed directly to the writing of this document:

Kevork N.~Abazajian (University of California, Irvine),
Peter Adshead (University of Illinois, Urbana-Champaign),
James Aguirre (University of Pennsylvania),
Zeeshan Ahmed (SLAC National Accelerator Laboratory),
Simone Aiola (Princeton University),
Yacine Ali-Haimoud (Johns Hopkins University),
Steven W.~Allen (Stanford University),
David Alonso (University of Oxford),
Adam Anderson (Fermilab National Accelerator Laboratory),
James Annis (Fermilab National Accelerator Laboratory),
John W.~Appel (Johns Hopkins University),
Douglas E.~Applegate (University of Chicago),
Kam S.~Arnold (University of California, San Diego),
Jason E.~Austermann (National Institute of Standards and Technology),
Carlo Baccigalupi (Scuola Internazionale Superiore di Studi Avanzati, Trieste, Italy),
Darcy Barron (University of California, Berkeley),
James G.~Bartlett (Laboratoire AstroParticule et Cosmologie - Université Paris Diderot, France),
Ritoban Basu Thakur (University of Chicago),
Nicholas Battaglia (Princeton University),
Daniel Baumann (Cambridge University),
Karim Benabed (Institut d'Astrophysique de Paris - Université Pierre et Marie Curie /  Centre National de la Recherche Scientifique, France),
Amy N.~Bender (Argonne National Laboratory),
Charles L.~Bennett (Johns Hopkins University),
Bradford A.~Benson (Fermilab),
Colin A.~Bischoff (University of Cincinnati),
Lindsey Bleem (Argonne National Laboratory),
J.~Richard Bond (Canadian Institute For Theoretical Astrophysics),
Julian Borrill (Berkeley Lab),
François R.~Bouchet (Institut d'Astrophysique de Paris),
Michael L.~Brown (University of Manchester),
Christopher Brust (Perimeter Institute),
Victor Buza (Harvard University),
Karen Byrum (Argonne National Laboratory),
Giovanni Cabass (University of Rome La Sapienza),
Erminia Calabrese (University of Oxford),
Robert Caldwell (Dartmouth College),
John E.~Carlstrom (University of Chicago),
Anthony Challinor (University of Cambridge),
Clarence L.~Chang (Argonne National Laboratory),
Hsin C.~Chiang (University of KwaZulu-Natal),
David T.~Chuss (Villanova University),
Asantha Cooray (University of California, Irvine),
Nicholas F.~Cothard (Cornell University),
Thomas M.~Crawford (University of Chicago),
Brendan Crill (Jet Propulsion Laboratory),
Abigail Crites (Caltech),
Francis-Yan Cyr-Racine (Department of Physics, Harvard University),
Francesco De Bernardis (Cornell University),
Paolo M.~de Bernardis (Physics Department Sapienza University),
Tijmen de Haan (University of California, Berkeley),
Jacques Delabrouille (Centre National de la Recherche Scientifique, France),
Marcel Demarteau (Argonne National Laboratory),
Mark Devlin (University of Pennsylvania),
Sperello di Serego Alighieri (INAF - Osservatorio Astrofisico di Arcetri),
Eleonora di Valentino (IAP),
Clive Dickinson (The University of Manchester),
Matt Dobbs (McGill University),
Scott Dodelson (Fermilab),
Olivier Dore (JPL/Caltech),
Joanna Dunkley (Princeton University),
Cora Dvorkin (Harvard University),
Josquin Errard (Institut Lagrange Paris),
Thomas Essinger-Hileman (Johns Hopkins University), 
Giulio Fabbian (Scuola Internazionale Superiore di Studi Avanzati, Trieste, Italy),
Stephen Feeney (Center for Computational Astrophysics),
Simone Ferraro (University of California, Berkeley),
Jeffrey P.~Filippini (University of Illinois at Urbana-Champaign),
Raphael Flauger (University of California, San Diego),
Aurelien A.~Fraisse (Princeton University),
George M.~Fuller (University of California, San Diego),
Patricio A.~Gallardo (Department of Physics, Cornell University.),
Silvia Galli (Institut d'Astrophysique de Paris),
Jason Gallicchio (Harvey Mudd),
Ken Ganga (APC),
Enrique Gaztanaga (Institute of Space Sciences),
Martina Gerbino (OKC, Stockholm University),
Mandeep S.~S.~Gill (Stanford),
Yannick Giraud-Héraud (APC - France),
Vera Gluscevic (Institute for Advanced Study),
Sunil Golwala (Caltech),
Krzysztof M.~Gorski (Jet Propulsion Laboratory),
Daniel Green (University of California, Berkeley),
Daniel Grin (Haverford College),
Evan Grohs (University of Michigan),
Riccardo Gualtieri (University of Illinois at Urbana Champaign),
Jon E.~Gudmundsson (Stockholm University),
Grantland Hall (Harvard University),
Mark Halpern (University of British Columbia),
Nils W.~Halverson (University of Colorado Boulder),
Shaul Hanany (University of Minnesota),
Shawn Henderson (Cornell University),
Jason W.~Henning (University of Chicago),
Sophie Henrot-Versille (LAL),
Sergi R.~Hildebrandt (California Institute of Technology),
J. Colin Hill (Columbia University),
Christopher M.~Hirata (The Ohio State University),
Eric Hivon (IAP),
Ren\'{e}e Hlo\v{z}ek (Dunlap Institute),
Gilbert Holder (University of Illinois at Urbana-Champaign),
William Holzapfel (University of California),
Wayne Hu (University of Chicago),
Johannes Hubmayr (NIST),
Kevin M.~Huffenberger (Florida State University),
Kent Irwin (Stanford),
Bradley R.~Johnson (Columbia University),
William C.~Jones (Princeton University),
Marc Kamionkowski (Johns Hopkins University),
Brian Keating (University of California, San Diego),
Sarah Kernasovskiy (Stanford University),
Reijo Keskitalo (Lawrence Berkeley Lab),
Theodore Kisner (Lawrence Berkeley National Laboratory),
Lloyd Knox (UC Davis),
Brian J.~Koopman (Cornell University),
Arthur Kosowsky (University of Pittsburgh),
John Kovac (Harvard University),
Ely D.~Kovetz (Johns Hopkins University),
Nicoletta Krachmalnicoff (Scuola Internazionale Superiore di Studi Avanzati, Trieste, Italy),
Chao-Lin Kuo (SLAC),
Akito Kusaka (Lawrence Berkeley National Laboratory),
Nicole A.~Larsen (University of Chicago),
Massimiliano Lattanzi (Università di Ferrara),
Charles R.~Lawrence (JPL),
Maude Le Jeune (Laboratoire AstroParticule et Cosmologie, Université Paris Diderot, France),
Adrian T.~Lee (University of California, Berkeley),
Antony Lewis (University of Sussex),
Marc Lilley (IAP),
Thibaut Louis (IAP),
Marilena Loverde (Stony Brook University),
Amy Lowitz (University of Wisconsin - Madison),
Philip M.~Lubin (UC Santa Barbara - Physics),
Juan J.~F.~Macias-Perez (LPSC),
Mathew S.~Madhavacheril (Princeton University),
Adam Mantz (Stanford University),
David J.~E.~Marsh (King's College London),
Silvia R.~M.~Masi (Physics Department Sapienza University),
Philip Mauskopf (Arizona State University),
Jeffrey McMahon (University of Michigan),
Pieter Daniel Meerburg (CITA),
Alessandro Melchiorri (University of Rome Sapienza),
Jean-Baptiste Melin (CEA Saclay),
Stephan Meyer (University of Chicago),
Joel Meyers (CITA),
Amber D.~Miller (University of Southern California),
Laura M.~Mocanu (University of Chicago),
Lorenzo Moncelsi (California Institute of Technology),
Julian B.~Munoz (Johns Hopkins University),
Andrew Nadolski (University of Illinois, Urbana-Champaign),
Pavel Naselsky (Niels Bohr Institute),
Paolo Natoli (University of Ferrara),
Ho Nam Nguyen (Stony Brook University),
Michael D.~Niemack (Cornell University),
Stephen Padin (University of Chicago),
Luca Pagano (IAS - Orsay),
Lyman Page (Princeton University),
Robert Bruce Partridge (Haverford College),
Guillaume Patanchon (APC - France),
Timothy J.~Pearson (Caltech),
Marco Peloso (University of Minnesota),
Julien Peloton (University of Sussex),
Olivier Perdereau (LAL),
Laurence Perotto (LPSC-CNRS-France),
Francesco Piacentini (Sapienza - University of Rome),
Michel Piat (APC - France),
Levon Pogosian (Simon Fraser University),
Clement Pryke (University of Minnesota),
Benjamin Racine (University of Oslo),
Srinivasan Raghunathan (University of Melbourne),
Alexandra Rahlin (Fermilab),
Marco Raveri (University of Chicago),
Christian L.~Reichardt (The University of Melbourne),
Mathieu Remazeilles (University of Manchester),
Graca Rocha (Jet Propulsion Laboratory),
Natalie A.~Roe (LBNL),
Aditya Rotti (Florida State University),
John Ruhl (Case Western Reserve University),
Laura Salvati (University of Rome, Sapienza),
Emmanuel Schaan (Princeton University),
Marcel M.~Schmittfull (University of California, Berkeley),
Douglas Scott (University of British Columbia),
Neelima Sehgal (Stony Brook University),
Sarah Shandera (The Pennsylvania State University),
Christopher Sheehy (Brookhaven National Laboratory),
Blake D. Sherwin (University of California, Berkeley),
Erik Shirokoff (University of Chicago),
Eva Silverstein (Stanford University),
Sara M.~Simon (University of Michigan),
Tristan L.~Smith (Swarthmore College),
Michael Snow (High Precision Devices),
Lorenzo Sorbo (University of Massachusetts, Amherst),
Tarun Souradeep (IUCAA),
Suzanne T.~Staggs (Princeton University),
Antony A.~Stark (Smithsonian Astrophysical Observatory),
Glenn D.~Starkman (Case Western Reserve University),
George F.~Stein (Canadian Institute for Theoretical Astrophysics),
Jason R.~Stevens (Cornell),
Radek Stompor (APC/France),
Kyle T.~Story (Stanford),
Chris Stoughton (Fermilab),
Meng Su (MIT),
Aritoki Suzuki (University of California, Berkeley),
Grant P.~Teply (University of California, San Diego),
Peter Timbie (UW-Madison),
Jesse I.~Treu (Princeton University),
Matthieu Tristram (LAL - CNRS),
Gregory Tucker (Brown University),
Sunny Vagnozzi (Stockholm University),
Alexander van Engelen (CITA),
Eve M.~Vavagiakis (Cornell University),
Joaquin D.~Vieira (University of Illinois at Urbana-Champaign),
Abigail G.~Vieregg (University of Chicago, Dept. of Physics),
Sebastian von Hausegger (Niels Bohr Institute),
Benjamin D.~Wandelt (Institut d'Astrophysique de Paris),
Scott Watson (Syracuse University),
Nathan Whitehorn (University of California, Berkeley),
Edward J.~Wollack (NASA Goddard Space Flight Center),
W.~L.~Kimmy Wu (University of California, Berkeley),
Zhilei Xu (Johns Hopkins University),
Ki Won Yoon (SLAC),
Matias Zaldarriaga (Institute for Advanced Study).


==> tcilcomm.tex <==
% Macros used for TCI styles released with Scientific Word 1.1.
%Copyright (C) 1992-93 TCI Software Research, Inc.
\typeout{TCILCOMM Macros for TCI styles <08 Apr 93>.}
%
% Revisions:
% 08 Apr 93 - GP change line length to under 80 characters
% 30 Mar 92 - AO added \setmoremathsizes and hooks to, e.g. \@xpt,
%             for support of bold Greek
%
%%ltg added this to try to get 12pt to come through
%\DeclareOption{12pt}{\renewcommand\@ptsize{2}}
%%end ltg

\def\@ptoptions{%
 \let\@elt\relax\@for\@tempa:=\@optionlist\do{%
  \expandafter\let\expandafter\@tempb\csname ds@\@tempa\endcsname
  \expandafter\let\expandafter\@tempc\csname ds@11pt\endcsname
  \ifx\@tempb\@tempc\else
   \expandafter\let\expandafter\@tempc\csname ds@12pt\endcsname
   \ifx\@tempb\@tempc\else\let\@tempb\relax\fi
   \fi
  \@tempb
  }%
 }%
%
% read in style file, but only process the pt size options
%
\def\@ptoptinput#1{%
 \let\@save@optionlist\@optionlist
 \let\@save@options\@options
 \let\@options\@ptoptions
 %
 \input #1
 %
 \let\@optionlist\@save@optionlist
 \let\@options\@save@options
 }%
%
% the <21 Feb 92> version of letter.sty requires:
\ifx\undefined\reset@font
 \def\reset@font{}%
 \fi
%
% Change LaTeX
%
% Add command to append tokens
\newtoks\@temptokenb
\long\def\appdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokena\the\@temptokenb}%
 }%
\long\def\prepdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokenb\the\@temptokena}%
 }%
% Discard contents of \box\@cclv at beginning of document
\appdef\document{{\output{\setbox\z@\box\@cclv}\endgraf\null\eject}}%
% Fix mark register expansion
\def\leftmark{\expandafter\@leftmark\botmark{}{}{}\@nil}%
\def\rightmark{\expandafter\@rightmark\firstmark{}{}{}\@nil}%
\def\@leftmark#1#2#3\@nil{#1}%
\def\@rightmark#1#2#3\@nil{#2}%
%
%\show\raggedright
\newskip\raggedglue
\raggedglue\z@ plus20\p@ minus\z@
\def\raggedright{%
 \let\\=\@centercr\@rightskip\raggedglue\rightskip
 \@rightskip\leftskip\z@\parindent\z@
 }%
%
\def\@centercr{%
 \ifhmode\unskip\else\@badcrerr\fi\@@par
 \@ifstar{\penalty\@M\@xcentercr}{\@xcentercr}%
 }%
%
\def\traceoutput{\tracingoutput2\showboxbreadth\maxdimen
 \showboxdepth\maxdimen}%
%
\newcount\@hour\newcount\@minute\chardef\@x10\chardef\@xv60
\def\@time{%
  \@minute\time\@hour\@minute\divide\@hour\@xv
  \ifnum\@hour<\@x 0\fi\the\@hour:%
  \multiply\@hour\@xv\advance\@minute-\@hour
  \ifnum\@minute<\@x 0\fi\the\@minute
  }%
%
% change \@array to allow \par to mean something within its scope
%
\def\@array [#1]#2{%
 \setbox\@arstrutbox\hbox{\vrule height\arraystretch\ht
  \strutbox depth\arraystretch\dp\strutbox width\z@}%
 \@mkpream{#2}%
 \edef\@preamble{\halign\noexpand\@halignto\bgroup\tabskip
  \z@\@arstrut\@preamble\tabskip\z@\cr}%
 \let\@startpbox\@@startpbox\let\@endpbox\@@endpbox
 \if#1t\vtop\else\if#1b\vbox\else\vcenter\fi\fi
 \bgroup
  %\let\par\relax
  \let\@sharp##
  \let\protect\relax
  \lineskip\z@\baselineskip\z@
  \@preamble
 }%
%
% Expands to hex digit corresponding to the value of the argument
%
\def\hexnumber@#1{\ifnum#1<10 \number#1\else
 \ifnum#1=10 A\else\ifnum#1=11 B\else\ifnum#1=12 C\else
 \ifnum#1=13 D\else\ifnum#1=14 E\else\ifnum#1=15 F\fi\fi\fi\fi\fi\fi\fi}%
%
% define command to set more math sizes.
% Styles like Greekbf will hook in here.
%
\def\setmoremathsizes#1#2#3{}%
%
% define size switch addenda
%  Note: these choices agree with those in lfonts.tex, even if incorrect.
%
\prepdef\@vpt{\setmoremathsizes{fiv}{fiv}{fiv}}%
\prepdef\@vipt{\setmoremathsizes{six}{six}{six}}%
\prepdef\@viipt{\setmoremathsizes{sev}{fiv}{fiv}}%
\prepdef\@viiipt{\setmoremathsizes{egt}{six}{fiv}}%
\prepdef\@ixpt{\setmoremathsizes{nin}{six}{fiv}}%
\prepdef\@xpt{\setmoremathsizes{ten}{sev}{fiv}}%
\prepdef\@xipt{\setmoremathsizes{elv}{egt}{six}}%
\prepdef\@xiipt{\setmoremathsizes{twl}{egt}{six}}%
\prepdef\@xivpt{\setmoremathsizes{frtn}{ten}{sev}}%
\prepdef\@xviipt{\setmoremathsizes{svtn}{twl}{ten}}%
\prepdef\@xxpt{\setmoremathsizes{twty}{frtn}{twl}}%
\prepdef\@xxvpt{\setmoremathsizes{twty}{twty}{svtn}}%
%
% The \newfield command defines (like \newenvironment) a user syntax:
%
%   \newfield{foo}
%
% lets you write
%
%   \begin{foo}...\end{foo}
%
% but differs from \newenvironment in that TeX parses the entire content
% of the field and stores it in a macro \the@foo, and then executes \@do@foo.
%
% This means that the content of the field is actually more like an argument
% than the content of an environment. So \verb will not necessarily work
% within a field, and neither will \index. Caveat emptor.
%
% The default procedure for a field is to process its argument within a
% group.  If you want a field to simply store its data away, define its
% procedure to be synonymous with \@empty, as illustrated below.
%
\long\def\@readenvir#1#2\end{%
 \appdef\envirsofar{#2}%
 \@ifnextchar\bgroup{\@checkenvir{#1}}{\@envirenderr}%
 }%
%
\def\@envirenderr{%
 \@latexerr{\string\end\space not followed by environment name}\@eha
 }%
%
\def\@checkenvir#1#2{%
 \def\@tempa{#1}\def\@tempb{#2}%
 \ifx\@tempa\@tempb
  \ifx\envirsofar\@blankspace\let\envirsofar\@empty\fi
  \expandafter\let\csname the@#1\endcsname\envirsofar
  \def\@tempa{\csname @do@#1\endcsname}%
  \else
  \appdef\envirsofar{\end{#2}}%
  \def\@tempa{\@readenvir{#1}}%
  \fi
 \@tempa
 }%
%
\def\newfield#1#2{%
 \expandafter\@ifdefinable\csname#1\endcsname{%
  \expandafter\def\csname#1\endcsname{%
   \endgroup\let\envirsofar\@empty\@readenvir{#1}%
   }%
  \expandafter\let\csname the@#1\endcsname\@empty
  \expandafter\ifx\csname @do@#1\endcsname\relax
   \expandafter\def\csname @do@#1\endcsname{{\csname the@#1\endcsname}}%
   \fi
  }%
 }%
%
\def\@blankspace{ }% SciWord's nil field
%
\def\letparBL{\def\par{\\}}%
\def\letparSP{\def\par{\ }}%
\def\letparQD{\def\par{\quad}}%
\def\letparSL{\def\par{\hbox to1em{\hfil/\hfil}}}%
%
% When \par is processed in the page head, gobble up the rest of the
% argument.
\def\@gobblepar#1\@empty{}%
%
% Physical page size after trim
\newdimen\trimwidth
\newdimen\trimheight
\newdimen\botmargin
\newdimen\marginpartotal
%
\def\adjustpagemargin{% adjust \oddsidemargin by \marginpartotal
 \marginpartotal\marginparwidth\advance\marginpartotal\marginparsep
 \advance\oddsidemargin\marginpartotal
 }%
%
\def\settextheight{% calculate textheight constrained by:
 \textheight\trimheight
 \advance\textheight-\topmargin
 \advance\textheight-\headheight
 \advance\textheight-\headsep
 \advance\textheight-\footskip
 \advance\textheight-\botmargin
 }%
%
\def\vcenterpagemargin{% calculate \topmargin constrained by:
 \topmargin\trimheight
 \advance\topmargin-\textheight
 \advance\topmargin-\headheight
 \advance\topmargin-\headsep
 \advance\topmargin-\footskip
 \divide\topmargin\tw@\botmargin\topmargin
 }%
%
\def\centerpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \divide\oddsidemargin\tw@
 \evensidemargin\oddsidemargin
 \adjustpagemargin
 }%
%
\def\leftpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \advance\oddsidemargin-\evensidemargin
 \adjustpagemargin
 }%

